ULF: Unsupervised Labeling Function Correction using Cross-Validation for Weak Supervision

A cost-effective alternative to manual data labeling is weak supervision (WS), where data samples are automatically annotated using a predefined set of labeling functions (LFs), rule-based mechanisms that generate artificial labels for the associated classes. In this work, we investigate noise reduction techniques for WS based on the principle of k-fold cross-validation. We introduce a new algorithm ULF for Unsupervised Labeling Function correction, which denoises WS data by leveraging models trained on all but some LFs to identify and correct biases specific to the held-out LFs. Specifically, ULF refines the allocation of LFs to classes by re-estimating this assignment on highly reliable cross-validated samples. Evaluation on multiple datasets confirms ULF's effectiveness in enhancing WS learning without the need for manual labeling.

==> chapters/04_ws_with_cv.tex <==
\section{WSCrossWeigh and WSCleanLab}
\label{subsec:wscw}
\label{wscw}

% \input{table/06b_result_roberta_table}
% \input{table/06b_result_roberta_table_new_full}


In order to have suitable baselines, we consider two other cross-validation-based methods initially proposed to improve manual data annotations: CrossWeigh \cite{crossweigh}, and Cleanlab \cite{northcutt2021confident}.
For a more detailed comparison, we introduce extensions of these frameworks for the weakly supervised setting. 
In contrast to the original methods, our extensions leverage the LF information resulting in more accurate results.


%In this section, we present our extension of two frameworks, CrossWeigh \cite{crossweigh}, and Cleanlab \cite{northcutt2021confident}, initially proposed for denoising the manually annotated data, for weakly supervised settings with leveraging the information about matching LFs. 

%\subsection{Weakly Supervised CrossWeigh (WSCW)} \label{subsec:wscw}
CrossWeigh was proposed for tracing inconsistent labels in crowdsourced annotations for named entity recognition.
The algorithm traces the repeatedly mislabeled entities by training multiple models in a cross-validation fashion on different data subsets, comparing the predictions on unseen data with its crowdsourced labels and reweighting the conflicting ones. 
% Importantly, the samples with entities annotated in hold-out samples are excluded from the training sets in order to refrain the model from making easy predictions.
%As in the straight-forward $k$-fold cross-validation, the data is randomly split into $k$ folds used to build $k$ training and hold-out sets; the training samples that include the entities annotated in hold-out samples are additionally filtered out.
%Thus, each of the $k$ trained models makes predictions only for the entities unseen during the training.
%Thus, if an entity was constantly mislabeled by crowdworkers, the model trained without it would be rid of this confusion.   
% This approach seems to be promising for detecting the unreliable LFs in a similar way: if an erroneous LF systematically makes wrong annotations, a model trained on data without it will deduce the labels basing on the unseen LFs only, and the error will be traced and reduced. 
Our \textbf{Weakly Supervised CrossWeigh} (WSCW) splits the data with respect to the LFs (by Eq. \ref{eq:lfs_splitting}) and trains the $k$ separate models on ${X_{train_i}}$.
The labels $\hat y$ predicted by the trained model for the samples in ${X_{out_i}}$ are then compared to the initial noisy labels $\tilde y$. 
All samples $X_j$ where $\hat y_j \neq \tilde y_j$ are claimed to be potentially mislabeled; their influence is reduced in further training. 
The whole procedure of errors detection is performed $t$ times with different partitions to refine the results.
%The sample weights $w_{x_N}$ are then calculated as $w_{x_j}=\epsilon^{c_{j}}$, where $c_{j}$ is the number of times a sample $x_j$ was classified as mislabeled, $0 \leq c_j \leq t$, and $\epsilon$ is parameter.
More details are provided in Appendix \ref{sec:app_wscw}.


% \vspace*{5 pt}
% \begin{center}
%$L_{train_i} = \bigcup\limits_{l_j \in f_j} l_j$
%$l_j \in \{f_1, ..., f_{k-1}\}$, $j \neq i$
% $X_{train_i} =\{x_{j} \mid L_{x_{j}} \cap L_{test_i} =\emptyset, 1 \leq j \leq n\}$ TODO
% \end{center}
% \vspace*{5 pt}

% \vspace*{5 pt}
% \begin{center}
% $w_{x_i}=\epsilon^{c_{i}}$
% \end{center}
% \vspace*{5 pt}

%\subsection{Weakly Supervised Cleanlab (WSCL)} \label{wscw}

%The second method we introduce is \textbf{Weakly Supervised Cleanlab} (WSCL) - an adaptation of Cleanlab framework \cite{northcutt2021confident} for weak supervision. 
The Cleanlab framework allows to find erroneous labels by estimating the joint distribution between the noisy labels and out-of-sample labels calculated by $k$-fold cross-validation.
%The main idea of Cleanlab is also similar to $k$-fold cross-validation, but, in contrast to WSCW,
In our extension \textbf{Weakly Supervised Cleanlab} (WSCL), we follow a similar approach, but adapt it to the weak supervision the same way as in WSCW: the cross-validation sets $X_{train_i}$ and $X_{out_i}$ sets are built considering the matched LFs by Eq. \ref{eq:lfs_splitting} (WSCL \textsubscript {\textit{lfs}}) or Eq. \ref{eq:sgn_splitting} (WSCL \textsubscript {\textit{sgn}}). 
%now, not data samples, but the labeling functions $L$ are randomly split into $k$ folds $\{f_1, ..., f_k\}$ and used for building the $X_{train_i}$ and $X_{test_i}$ sets, $1 < i < k$, for training $k$ models ().
These sets are used to train $k$ models, which predict the class probabilities for the held-out samples, later transformed to the exact labels $\hat y$ concerning the class expected value. 
The correspondence between noisy and out-of-sample predicted labels determines the number of samples to be pruned
% is reflected in a class-to-class confident joint matrix $C_{K \times K}$, where $C [j][l]=|\{x_i \in X | y_i = j,\tilde y_i=l\}|$ 
(the same way as in the default setting of \citet{northcutt2021confident}).
Notably, Cleanlab counts the samples with presumably incorrect noisy labels $\tilde y$ only, but does not provide any estimate about what LFs assigned these noisy labels (in contrast to ULF). 
For more details, see Appendix \ref{sec:app_wscl}.

% A sample $x_i$ is considered to confidently belong to class $j\in K$ if the probability of class $j$ is greater than expected self-confidence for this class $t_{j}$ or the maximal one in case of several classes are probable. 
% The samples with no probability exceeding the thresholds have no decisive label and do not participate in the further denoising. 

%which predict the probability vector of class distribution ${\hat p(\hat y=j; x_i, \theta), j \in K}$ for each sample $x_i$ in the $X_{test_i}$.
%Next, for each sample $x_i$ in the $X_{test_i}$ the model predicts not the label, but the probability vector of class distribution ${\hat p(\hat y=j; x_i, \theta), j \in K}$.
%The labels $\hat y$ are calculated later on with respect to the class expected self-confidence value $t_j$ (see \cite{northcutt2021confident} for more details).

% \vspace*{-15 pt}
% \begin{gather}
%% $\large{T_k := \frac{\sum_{X_{k}} \hat{p}(y=k ; x_i, \theta)}{X_{k}} }$, \par
% \label{eq:threshold}
% \large{t_j := \frac{\sum_{X_j} % \hat{p}(y=j; x_i, \theta)}{|X_j|} },
% \end{gather}
% where $X_j = \{x_i \in X_{{y}=j}\}$ , $ 1 < j < c$

% \vspace*{-20 pt}
% \begin{gather}
% \label{eq:label_calc}
% \hat y_i=\argmax\limits_{{\substack{j \in[K]: \\ \hat{p}({y}=j ; x_i, \theta) \geq t_{j}}}} \hat{p}({y}=j ; x_i, \theta)
% \end{gather}


%but does not give us any insights about the erroneous of the corresponding labeling functions that assigned this noisy label to this sample (in contrast to the ULF approach we present in Section \ref{sec:ulf}). 

%The confident matrix $C$ is then calibrated and normalized in order to obtain an estimate matrix of the joint distribution between noisy and predicted labels $\hat Q_{K \times K}$, which determines the number of samples to be pruned.
%We perform the pruning by noise rate following the Cleanlab default setting: $n \cdot \hat Q, i \neq j$ samples with $max(\hat p(y = j)- \hat p(y = i))$ are eliminated in further training.
%are the samples with the noisy label $y^ = k_i$ maximal difference between the probability of a given label $\hat y$ and the maximal probability of non-given labels is the largest. The missing data is compensated by recalculating the sample weights. 

% \begin{table*}[ht]
% \centering
% \caption{Statistics of all the dataset.}
% \label{tab:data}
% \begin{tabular}[t]{lcccccc}
% \toprule
%  & \textbf{#Train / #Test} & \textbf{\#Classes} & \textbf{\#Rules} & \textbf{Average Rules Hits}  & \textbf{Rule Accuracy} \\
% \midrule
% YouTube & 1586/250 & 2 & 10 & 1.62 & \\
% Spouse & 22254/2701 & 2 & 9 & 33.7 \\
% TREC & 4965/500 & 6 & 68 & 1.73 & \\
% SMS & 4502/500 & 2 & 73 & 0.509 & \\
% \bottomrule
% \end{tabular}
% \end{table*}

==> pseudocode/ulf_cosine_pseudocode.tex <==
\LinesNotNumbered

\begin{algorithm}[h!]
\caption{Train ($\theta$, $X$, $\tilde Y$): DeepULF; pretrained language model fine-tuning (optionally: with Cosine self-training)}
\label{alg:ulf_cosine}
\SetAlgoLined
\SetKwInOut{KwReturn}{Output} % set the Output
    % \State \hskip1.8em \textit{\# fine-tune $\theta$ with $X$ and $Y_n$}\\
\nextnr
$X_{lab}$ = $\{x \in X : |L_{x_i}| > 0 \}$ \\
\nextnr
$\tilde Y_{lab}$ = $\{\tilde y \in \tilde Y : \forall x \in X_{lab}\}$ \\
\textit{\# 1. fine-tune $\theta$ with $X_{lab}$ and $\tilde Y_{lab}$}\\
\nextnr
{$\theta$} = AdamW($\theta$, $X_{lab}$, $\tilde Y_{lab}$) \\
\textit{\# 2. (optional) contrastive self-training of $\theta$ with $X$}\\
\nextnr
Calculate pseudo labels ${y \textsubscript{psd}}$ \\
\nextnr
\For{step = 1, 2, ..., num\_steps}{
    \nextnr
    Select confident samples \\
    \nextnr
    Calculate classification loss $L_c(\theta, y \textsubscript{psd})$,  contrastive regularizer $R_1(\theta, y \textsubscript{psd})$, and confidence resularizer $R_1(\theta)$ \\
    \nextnr
    $L(\theta, y \textsubscript{psd}) = L_c + \lambda R_1 + R_1$ \\
    \nextnr
    \State {$\theta$} = AdamW($\theta$, $X$) \\
}
\KwReturn{Trained $\theta$}
\end{algorithm}
% \vspace{-1em}

==> pseudocode/ulf_logreg_pseudocode.tex <==
\begin{algorithm}[h]
\caption{Train ($\theta$, $X$, $\tilde Y$):\\ Feature-based ULF}
\label{alg:ulf_logreg}
\SetAlgoLined
\SetKwInOut{KwReturn}{Output} % set the Output
    %\State \hskip1.8em {$\hat \theta$} = AdamW($\theta$, $X$, $Y_n$) \\
\State{$\theta$} = AdamW($\theta$, $X$, $\tilde Y$) \\
\KwReturn{Trained {$\theta$}}
\end{algorithm}

==> pseudocode/ulf_pseudocode.tex <==
\SetAlgoLined

\begin{algorithm}[h]
\caption{ULF: Unsupervised Labeling Function Correction for Weak Supervision}
\label{alg:ulf}
\SetKwInput{KwIn}{Input}    % Set the Input
\SetKwInOut{KwReturn}{Output} % set the Output
\DontPrintSemicolon
\KwIn{unsupervised training data~$X$, \newline samples to LFs matrix~$Z_{N \times L}$, \newline LFs to classes matrix~$T_{L \times K}$}
%Collect set of signatures S, S_i = {L_{x_i}}  \\
Calculate noisy labels $\tilde Y \leftarrow Z * T$  \\
\For{$iter = 1, 2, ... I$}{
    Randomly split LFs $L$ or signatures $\bigcup {L_{x_i}}$ into \textit{k} folds ${f_1, ..., f_k}$  \\
    \For{f = 1, 2, ..., k} {
        Build $X_{train_i}$, $X_{test_i}$ sets (Eq. \ref{eq:lfs_splitting}, \ref{eq:sgn_splitting})  \\
        $\tilde Y_{train_i} = \{\tilde y \in \tilde Y : \forall x \in X_{train_i}\}$ \\
        % Train model $\theta{_i}$ using~$X_{train_i}$ and $Y_n$  \\
        Train ($\theta{_i}$, $X_{train_i}$, $\tilde Y_{train_i}$)  \\
        Calculate ${p(\tilde y=j; x_i, \theta_i)}$ 
    }  
    Get labels $\hat y_i$ (Eq.~\ref{eq:label_calc}) with respect to the thresholds $t_j$  \\
    Calculate LFs-to-class confident matrix $C_{l,\hat y}$ (Eq.~\ref{eq:conf_matrix}) \\
    Estimate a joint matrix $\hat Q_{l, \hat y}$ (Eq.~\ref{eq:calibr}) \\
    Recalculate $T^{\ast}$ matrix (Eq.~\ref{eq:t_recalc}) \\
    Calculate new noisy labels $\tilde Y^{\ast}$ with  $T^{\ast}$
}
% Train model $\theta$ with ~$X_{train_i}$ and $Y_n$ \\
Train ($\theta$, $X$, $\tilde Y^{\ast}$) \\
\KwReturn{Trained $\theta$}
\end{algorithm}

\vspace*{-2pt}

==> table/ablation_study.tex <==
\begin{table}[ht]
\scriptsize
\renewcommand\arraystretch{1.5}
\centering
\begin{tabularx}{\columnwidth}{@{\extracolsep{\fill}} l|c|c|c|c}
\toprule
%& \multicolumn{2}{l}\textbf{\textbf{\thead{YouTube \\ (Acc)}}} | & \multicolumn{2}{l}{\textbf{\thead{Spouse \\ (F1)}} } | & \multicolumn{2}{l}{\textbf{\thead{TREC \\ (Acc)}}} | & \multicolumn{2}{l}{\textbf{\thead{SMS \\ (F1)}}} \\

%& \textbf{\textbf{\thead{\tiny{YouTube (Acc)}}}} & \textbf{\thead{\tiny{Spouse (F1)}}} & 
%\textbf{\thead{\tiny{TREC (Acc)}}} & 
%\textbf{\thead{\tiny{SMS (F1)}}} \\

& \textbf{\thead{\scriptsize{YouTube} \\ \scriptsize{(Acc)}}} & 
\textbf{\thead{\scriptsize{Spouse} \\ \scriptsize{(F1)}}} & 
\textbf{\thead{\scriptsize{TREC} \\ \scriptsize{(Acc)}}} & 
\textbf{\thead{\scriptsize{SMS} \\ \scriptsize{(F1)}}} \\



\midrule
\midrule
%& {\scriptsize LogReg} & {\scriptsize RoBerta} & {\scriptsize LogReg} & {\scriptsize RoBerta} & {\scriptsize LogReg} & {\scriptsize RoBerta} & {\scriptsize LogReg} & {\scriptsize RoBerta} \\
%Majority & $82.3 \pm 0.8$ & $44.0 \pm 0.6$ & $60.9 \pm 0.4$ & $54.5 \pm 1.8$ % & $65.0 \pm 0.2$ \\
DeepULF& 
\normal{96.8} & 
\normal{} & 
\normal{76.8} & 
\normal{}
\\
FT + FT& 
\normal{94.4} & 
\normal{} & 
\normal{55.8} & 
\normal{} 
\\
FT + Cos& 
\normal{88.8} & 
\normal{} & 
\normal{75.4} & 
\normal{} 
\\
Cos + FT& 
\normal{95.6} & 
\normal{} & 
\normal{49.2} & 
\normal{} 
\\
\bottomrule
\end{tabularx}
\caption{DeepULF: Ablation study.}
\label{tab:results}
\end{table}
\footnotetext{The trained model will be publicly released on acceptance.}


==> table/case_study.tex <==
\begin{table*}
\centering
\small
\begin{tabular}[t]{cllccc}
\toprule
 & \textbf{Sample} 
 & \textbf{LFs matched} 
 & \textbf{Noisy Label} 
 & \textbf{Corrected Label} 
 & \textbf{Gold Label}
 \\ % & \textbf{IMDb}\\
\midrule
1 & 
Hello! I'm Marian, I'm a singer from Venezuela! I was part of a boy-girl band named cubik, and I'm now singing on my own 'cause I wanted to play my own pop and pop-rock songs. It would mean a lot if you could have a look at my channel to check my music and watch my new video!! and if u like, subscribe to it! XOXO THANKS!! & keyword_my, keyword_subscribe, keyword_song, textblob_subjectivity & 
HAM & 
SPAM & 
SPAM \\       % & 40000
\bottomrule
\end{tabular}
\end{table*}[ht]

==> table/ulf_combi.tex <==
\begin{table*}[h]
%\vspace*{-5pt}
\centering
%\renewcommand\arraystretch{1.2}
\begin{tabular}{lcccc|c}  
%{@{\hspace{0.08cm}}l@{\hspace{0.08cm}}l@{\hspace{0.08cm}}cc@{\hspace{0.08cm}}cc@{\hspace{0.08cm}}|c}
\toprule
& \textbf{YouTube \small{(Acc)}} &
\textbf{Spouse \small{(F1)}}& 
\textbf{TREC \small{(Acc)}} & 
\textbf{SMS \small{(F1)}} & 
\textbf{Avg}\\[-0.3em]
\midrule
\midrule
WSCrossWeigh & 
90.8 \small{$\pm$ 0.7} & 
42.0 \small{$\pm$ 0.0} &
46.0 \small{$\pm$ 0.4} &
84.0 \small{$\pm$ 0.9} & 
65.7
\\[-0.0em]
WSCleanlab \textsubscript {\textit{lfs}} & 
87.2 \small{$\pm$ 0.4} & 
44.4 \small{$\pm$ 0.7} & 
58.9 \small{$\pm$ 0.3} & 
86.6 \small{$\pm$ 0.3} &
69.3
\\[-0.0em]
WSCleanlab \textsubscript {\textit {sgn}} & 
88.3 \small{$\pm$ 0.5} & 
44.6 \small{$\pm$ 0.9} &
56.4 \small{$\pm$ 0.3} &
85.1 \small{$\pm$ 0.3} & 
68.6
\\[-0.0em] 
\hline
ULF \textsubscript {\textit {rndm}} &
92.8 \small{$\pm$ 0.1} & 
44.8 \small{$\pm$ 0.5} & 
58.0 \small{$\pm$ 0.2} &
85.7 \small{$\pm$ 0.5} & 
70.3
\\
% ULF \textsubscript {\textit {rndm} w/ prior & 92.7 $\pm$ 1.1 & -- & -- & 85.1 $\pm$ 2.0 \\
ULF \textsubscript {\textit {lfs}} &
90.8 \small{$\pm$ 0.9} &
44.0 \small{$\pm$ 0.9} &
55.5 \small{$\pm$ 0.4} &
70.0 \small{$\pm$ 0.4} &
65.1
\\
% ULF \textsubscript {\textit {lfs}} w/ prior & 90.5 $\pm$ 3.2  & -- & -- & \color{red}{70.0 $\pm$ 0.8} \\
% ULF \textsubscript {\textit {sgn}} w/ prior & 93.7 $\pm$ 0.6  & -- & -- & 88.4 $\pm$ 1.8 \\
ULF \textsubscript {\textit {sgn}} & 
\textbf{94.6} \small{$\pm$ 0.2} & 
\textbf{49.8 \small{$\pm$ 1.0}} & 
58.2 \small{$\pm$ 0.2} &
\textbf {88.6} \small{$\pm$ 0.3} & 
\textbf{72.8} \\[-0.0em]
\bottomrule
\end{tabular}
\caption{Feature-based ULF results
%The best results are marked \textbf{bold}, the second best - \underline{underlined}. 
averaged over 10 trials and reported with the standard error of the mean. 
The results marked with * are taken directly from \citet{zhang2021wrench}. 
% \vspace{0pt}[1] - \citealt{snorkel}, [2] - \citealt{crossweigh}, [3] - \citealt{northcutt2021confident}
}
%\vspace*{-14pt}
\label{tab:ulf_full_results}
\end{table*}
